Policy Optimization as Online Learning with Mediator Feedback

Policy Optimization (PO) is a widely used approach to address continuous control tasks. In this paper, we introduce the notion of mediator feedback that frames PO as an online learning problem over the policy space. The additional available information, compared to the standard bandit feedback, allows reusing samples generated by one policy to estimate the performance of other policies. Based on this observation, we propose an algorithm, RANDomized-exploration policy Optimization via Multiple Importance Sampling with Truncation (RANDOMIST), for regret minimization in PO, that employs a randomized exploration strategy, differently from the existing optimistic approaches. When the policy space is finite, we show that under certain circumstances, it is possible to achieve constant regret, while always enjoying logarithmic regret. We also derive problem-dependent regret lower bounds. Then, we extend RANDOMIST to compact policy spaces. Finally, we provide numerical simulations on finite and compact policy spaces, in comparison with PO and bandit baselines.

==> plot_style.tex <==
%\usepakage{xcolor}

\definecolor{brightBlue}{RGB}{68, 119, 170}
\definecolor{brightCyan}{RGB}{102, 204, 238}
\definecolor{brightGreen}{RGB}{34, 136, 51}
\definecolor{brightYellow}{RGB}{204, 187, 68}
\definecolor{brightRed}{RGB}{238, 102, 119}
\definecolor{brightPurple}{RGB}{170, 51, 119}
\definecolor{brightGrey}{RGB}{187, 187, 187}

\definecolor{vibrantBlue}{RGB}{0, 119, 187}
\definecolor{vibrantCyan}{RGB}{51, 187, 238}
\definecolor{vibrantTeal}{RGB}{0, 153, 136}
\definecolor{vibrantOrange}{RGB}{238, 119, 51}
\definecolor{vibrantRed}{RGB}{204, 51, 17}
\definecolor{vibrantMagenta}{RGB}{238, 51, 119}
\definecolor{vibrantGrey}{RGB}{100, 100, 100}

\tikzstyle{dotted}=                  [dash pattern=on \pgflinewidth off 2pt]
\tikzstyle{densely dotted}=          [dash pattern=on \pgflinewidth off 1pt]
\tikzstyle{loosely dotted}=          [dash pattern=on \pgflinewidth off 4pt]

\tikzstyle{dashed}=                  [dash pattern=on 3pt off 3pt]
\tikzstyle{densely dashed}=          [dash pattern=on 3pt off 2pt]
\tikzstyle{loosely dashed}=          [dash pattern=on 3pt off 6pt]

\tikzstyle{dashdotted}=              [dash pattern=on 3pt off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dashdotted}=      [dash pattern=on 3pt off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dashdotted}=      [dash pattern=on 3pt off 4pt on \pgflinewidth off 4pt]

\tikzstyle{dash dot dot}=[dash pattern=on 3pt off 2pt on \pgflinewidth off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dash dot dot}=[dash pattern=on 3pt off 1pt on \pgflinewidth off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dash dot dot}= [dash pattern=on 3pt off 4pt on \pgflinewidth off 4pt on \pgflinewidth off 4pt]

\tikzstyle{dash dash dot}=[dash pattern=on 3pt off 2pt on 3pt off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dash dash dot}=[dash pattern=on 3pt off 1pt on 3pt off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dash dash dot}= [dash pattern=on 3pt off 4pt on 3pt off 4pt on \pgflinewidth off 4pt]

\tikzstyle{dash dash dot dot}=[dash pattern=on 3pt off 2pt on 3pt off 2pt on \pgflinewidth off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dash dash dot dot}=[dash pattern=on 3pt off 1pt on 3pt off 1pt on \pgflinewidth off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dash dash dot dot}= [dash pattern=on 3pt off 4pt on 3pt off 4pt on \pgflinewidth off 4pt on \pgflinewidth off 4pt]

\pgfplotsset{
	cycle list/.define={vibrant}{
    	vibrantBlue, solid, every mark/.append style={solid, fill=vibrantBlue},mark=*\\
    	vibrantCyan, densely dashed, every mark/.append style={solid, fill=vibrantCyan}, mark=triangle*\\
    	vibrantTeal, densely dotted, every mark/.append style={solid, fill=vibrantTeal}, mark=square*\\
    	vibrantOrange, densely dashdotted, every mark/.append style={solid, fill=vibrantOrange}, mark=diamond*\\
        vibrantRed, densely dash dot dot, every mark/.append style={solid, fill=vibrantRed, scale=1.5}, mark=x\\
        vibrantMagenta, densely dash dash dot, every mark/.append style={solid, fill=vibrantMagenta, scale=1.5}, mark=star\\
        vibrantGrey, densely dash dash dot dot, every mark/.append style={solid, fill=vibrantGrey, scale=1.5}, mark=|\\
        },
    }
